A Weak Formulation of Water Waves in Surface Variables

In this short note, we derive a system of two nonlocal equations for the water-wave problem following the work of [AFM06]. Specifically, we consider a fluid with a one-dimensional free surface for an irrotational fluid both with, and without, surface tension. We show that these equations can be useful for deriving direct maps between boundary data at the various interfaces and consider various asymptotic regimes. Finally, for periodic traveling wave solutions, we derive a new single-equation that is derivative free and has the potential to simplify the process of finding asymyptotic expansions of the solutions as well as reduce numerical errors when solving computationally.

==> sections/constant_vorticity.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Constant vorticity}
    \begin{figure}[htp]
        \centering
        \psset{xunit=.5in,yunit=.3in,plotpoints=200,plotstyle=line}
        \begin{pspicture}(-6,-1)(6,1.75)
            \psaxes[linewidth=.1pt, labels=all]{->}(-5.5,-1.4)(-5.5,-1.4)(-5.2,-.8)[$x$,-90][$z$,-180]
            % Plot the fluid domain
            \plotWave{2}{0}{25}

            % Plot Arrows
            
            \psline[linestyle = dashed,linecolor=black!80,linewidth=.4pt](-2.95,0)(-2.95,-1)
            \psline[linestyle = dashed,linecolor=black!80,linewidth=.4pt](-3.25,0)(-4.25,-1)
            \multido{\iX=0+1,\iY=1+1}{4}{%
	            \psline[arrows=->,linestyle=solid,linewidth=.4pt,linecolor=black]%
		        (\fpeval{-3},\fpeval{-(1)/5*(\iY)})%
                (\fpeval{-\iX/5-3.4},\fpeval{-(1)/5*(\iY)})}
            % Plot the bottom
            \pscustom[linestyle=none,fillstyle=solid,fillcolor=black!30,algebraic=true]{%
                \psplot{-5}{5}{-1}%
                \psplot{5}{-5}{-1.2 } 
                } 
            \psplot[algebraic=true,linewidth=.4pt]{-5}{5}{-1}
            % Plot the axes
            %\psaxes[ticks=none,labels=none,arrowscale=2,linewidth=.6pt,linecolor=black!80]{->}(-5,0)(-5,-1.2)(5.25,1.5)
            \uput[d](0,0){$\mathscr{D}$}
            \uput[r](5,-1){$z = -h$}
            \uput[r](5,0){$z = \eta(x,t)$}
        \end{pspicture}
        \caption{Fluid Domain for Constant Vorticity}
    \end{figure}
    As discussed in \cite{ashton2011non}, the formulation given by \cite{ablowitz2006new} can be extended to include constant vorticity.  We are able to do the same following a similar process.  We begin by considering the equations of motion expressed in terms of the fluid velocities given by 
    \begin{align}
        &u_x + v_z = 0, &&(x,z)\in \mathscr{D},\label{eqn:conMassCV}\\
        &v_x - u_z = \omega, &&(x,z) \in \mathscr{D},\label{eqn:CV}\\
        &u_t + \left(\frac{1}{2}(u^2 + v^2) + gz + p\right)_x -\omega v = 0, &&(x,z)\in \mathscr{D}\label{eqn:uB}\\
        &v_t + \left(\frac{1}{2}(u^2 + v^2) + gz + p\right)_z +\omega u = 0, &&(x,z)\in \mathscr{D}\label{eqn:vB}\\
        &v = 0, && z= -h\label{eqn:kinematicBottomCV}\\
        &\eta_t = v - \eta_x u && z= \eta,\label{eqn:kinematicCV}\\
        &p = 0, && z= \eta, \label{eqn:pressureBC}
    \end{align} 
    where $\omega$ is a constant throughout the fluid.  Since we are considering the case of constant vorticity, then following \cite{wahlen2007hamiltonian,ashton2011non}, we can use a streamfunction formulation where we define 
    \begin{displaymath}
        \tpsi = \psi + \frac{\omega}{2}z^2\quad \to\quad \nabla\tpsi = \nabla\psi + \begin{bmatrix}0\\\omega z\end{bmatrix} = \begin{bmatrix}-v\\u + \omega z\end{bmatrix}.
    \end{displaymath}
    With this definition, it is clear the $\tpsi$ is harmonic. Likewise, we can introduce $\phi$ as the harmonic conjugate of $\tpsi$ such that
    \begin{displaymath}
        \nabla\phi = \begin{bmatrix}u+\omega z\\v\end{bmatrix}.
    \end{displaymath}
    \hl{Say something about the far-field boundary conditions on $\phi$ and $q$}
    Following the work of \cite{gavrilyuk2015kinematic}, we also introduce the generalized potential function $q(x,t)$ such that $q_x = u + \eta_x v,$ along the free-surface $z = \eta$.  With this variable, we can rewrite \eqref{eqn:pressureBC} as 
    \begin{equation}
        q_t +\frac{1}{2}u^2 - \frac{1}{2}v^2+uv\eta_x + g\eta=0, \quad z = \eta,\label{eqn:conVortQT}
    \end{equation}
    where we have set the integration constant to be zero by assuming that a coordinate systems is chosen so that $q \to 0$ as $\vert x \vert \to \infty$.  The variables $q$ and $\phi$ are related via the expression 
    \begin{displaymath}
        q_x = \frac{d}{dx}\phi(x,\eta,t) - \omega\eta, \quad \to \quad q = \phi(x,\eta,t) - \partial_x^{-1}\left(\omega\eta\right).
    \end{displaymath}  
    It will also be useful to note that along the free-surface $z = \eta$, that 
    \begin{displaymath}
        \nabla\phi\dotn = v - \eta_x u - \omega\eta\eta_x = \eta_t-\omega\eta\eta_x, \quad \nabla\phi\dott =  u + \eta_xv + \omega\eta,
    \end{displaymath}
    modulo some arbitrary function of time.

    \subsection{Derivation of the Nonlocal/Nonlocal Formulation}
        Since $\phi$ is harmonic in the fluid domain, we can follow exactly the same process as outlined in \Cref{ssec:derivation1d}. This yields the following nonlocal/nonlocal formulation
        \begin{equation}
            \sint{(\eta_t - \omega\eta\eta_x)\varphi_z - (q_x+ \omega\eta)\varphi_x} = -\bint{(u - \omega h)\varphi_x}
        \end{equation}
        \begin{equation}
            \sint{\varphi_{zz}\left(\omega\eta q_x - g\eta - q_t - \frac{1}{2}(\omega\eta)^2\right) + \varphi_{xz}\left(\frac{\omega^2}{2}\eta^2\eta_x - g\eta\eta_x + q_x\eta_t - \eta_xq_t + \omega\eta\eta_t\right)} = \bint{u_x(u - \omega h)\varphi_x}
        \end{equation}


==> sections/multi_layer_flows.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Multiple fluid layers}        
    \begin{figure}[htp]
        \centering
        \psset{xunit=.5in,yunit=.3in,plotpoints=200,plotstyle=line}
        \begin{pspicture}(-6,-1)(6,3.75)
            \plotWave{2}{1.5}{10}
            \plotWave{0}{.75}{20}
            \plotWave{-4}{-.5}{40}
            \uput[r](5,1.5){$z =\eta_1(x,t)$}
            \uput[r](5,.75){$z =\eta_2(x,t)$}
            \uput[r](5,.25){$\vdots$}
            \uput[r](5,-.5){$z =\eta_n(x,t)$}
            \uput[r](5,-1.25){$z =0$}

            \uput[r](-4.5,1.125){$\rho_1, \phi_1, \mathscr{D}_1$}
            \uput[r](-4.5,.25){$\vdots$}
            \uput[r](-4.5,-.75){$\rho_n, \phi_n, \mathscr{D}_n$}
            % Plot the bottom
            \pscustom[linestyle=none,fillstyle=solid,fillcolor=black!20,algebraic=true]{%
                \psplot{-5}{5}{-1.25}%
                \psplot{5}{-5}{-1.45 } 
                } 
            \psplot[algebraic=true,linewidth=.4pt]{-5}{5}{-1.25}
            % Plot the axes
            %\psaxes[ticks=none,labels=none,arrowscale=2,linewidth=.6pt,linecolor=black!80]{->}(-5,0)(-5,-1.2)(5.25,1.5)
            %\uput[d](0,0){$\mathscr{D}$}
            
        \end{pspicture}
        \caption{Fluid Domain for Multiple Fluid Layers}
    \end{figure}
    \begin{eqnarray}
        &&\dt\oint_{\partial\mathscr{D}_j}{\left[\varphi-\epsilon t \phi_j\normD{\varphi}\:ds\right]} =- \epsilon t\dt\oint_{\partial\mathscr{D}_j}\phi_j\normD{\varphi}\:ds\\    
        &&\dt\oint_{\partial\mathscr{D}_j}\phi_j\normD{\varphi_z}\:ds=\oint_{\partial\mathscr{D}_j}{\left[\left(\varphi_{zz}\dt(\phi_j) + \epsilon\varphi_{xz}\normD{\phi_j}\dx(\phi_j)\right)\:dx - \varphi_{xz}\dt(\phi_j)\:dz\right]}
    \end{eqnarray}
